Quantifying and Learning Static vs. Dynamic Information in Deep Spatiotemporal Networks

There is limited understanding of the information captured by deep spatiotemporal models in their intermediate representations. For example, while evidence suggests that action recognition algorithms are heavily influenced by visual appearance in single frames, no quantitative methodology exists for evaluating such static bias in the latent representation compared to bias toward dynamics. We tackle this challenge by proposing an approach for quantifying the static and dynamic biases of any spatiotemporal model, and apply our approach to three tasks, action recognition, automatic video object segmentation (AVOS) and video instance segmentation (VIS). Our key findings are: (i) Most examined models are biased toward static information. (ii) Some datasets that are assumed to be biased toward dynamics are actually biased toward static information. (iii) Individual channels in an architecture can be biased toward static, dynamic or a combination of the two. (iv) Most models converge to their culminating biases in the first half of training. We then explore how these biases affect performance on dynamically biased datasets. For action recognition, we propose StaticDropout, a semantically guided dropout that debiases a model from static information toward dynamics. For AVOS, we design a better combination of fusion and cross connection layers compared with previous architectures.

==> core/abstract.tex <==
Deep spatiotemporal models are used in a variety of computer vision tasks, such as action recognition and video object segmentation. Currently, there is a limited understanding of what information is captured by these models in their intermediate representations. For example, while it has been observed that action recognition algorithms are heavily influenced by visual appearance in single static frames, 
there is no quantitative methodology for evaluating such static bias in the latent representation compared to bias toward dynamic information (\eg motion).
We tackle this challenge by proposing a novel approach for quantifying the static and dynamic biases of any spatiotemporal model. To show the efficacy of our approach, we analyse two widely studied tasks, action recognition and video object segmentation. 
Our key findings are threefold: (i) Most examined spatiotemporal models are biased toward static information; although, certain two-stream architectures with cross-connections show a better balance between the static and dynamic information captured. (ii) Some datasets that are commonly assumed to be biased toward dynamics are actually biased toward static information. (iii) Individual units (channels) in an architecture can be biased toward static, dynamic or a combination of the two.


==> core/graphs/vos_arch_indiv_histograms.tex <==

\begin{figure*}[t]
\centering
%\begin{subfigure}{.33\textwidth}
%    \includegraphics[width=\textwidth]{tex/images/vos_joint_encoding_neurons/fseg/raw_layer4,sensor_fusion.png}
%    \caption{}
%\end{subfigure}%
%\begin{subfigure}{.33\textwidth}
%    \includegraphics[width=\textwidth]{tex/images/vos_joint_encoding_neurons/matnet/raw_layer4,sensor_fusion.png}
%    \caption{}
%\end{subfigure}%
%\begin{subfigure}{.33\textwidth}
%    \includegraphics[width=\textwidth]{tex/images/vos_joint_encoding_neurons/rtnet/raw_layer4,sensor_fusion.png}
%    \caption{}
%\end{subfigure}%

\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/fusionseg/app_fseg.png}
    \caption{}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/fusionseg/mot_fseg.png}
    \caption{}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/matnet/app_matnet.png}
    \caption{}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/matnet/mot_matnet.png}
    \caption{}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/rtnet/app_rtnet.png}
    \caption{}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=\textwidth]{tex/images/rtnet/mot_rtnet.png}
    \caption{}
\end{subfigure}

    \caption{Individual Units Analysis Histograms in (a,b) FusionSeg~\cite{jain2017fusionseg} modified and (c,d) MATNet~\cite{zhou2020motion} respectively. It shows the histogram for static (a,c) and dynamic (b,d) factors for both models. }
    \label{fig:vos_indiviual_units}
\end{figure*}

==> core/graphs/vos_dataset_astable.tex <==
\begin{figure} [t]
\begin{center}

% \resizebox{0.47\textwidth}{!}{

% \begin{tabular}{c |cc|cc|cc}
% \specialrule{1.2pt}{1pt}{1pt}

%  \multirow{2}{*}{Method}&  \multicolumn{2}{c}{\textbf{TAO-VOS}} & \multicolumn{2}{c}{\textbf{ImageNetVID}} &  \multicolumn{2}{c}{\textbf{TAO-VOS}}   \\
% %\hline
%   & Dyn.(\%) & Stat.(\%)& Dyn.(\%) & Stat.(\%)& Dyn.(\%) & Stat.(\%) \\
%     \specialrule{1.2pt}{1pt}{1pt}
%     	\specialrule{1.2pt}{1pt}{1pt}
% Sensor Fusion L5 & 26.4 & 25.8 & 26.4 & 33.1 & 27.8 & 30.1 \\ 
% Sensor Fusion L2 & 33.7 & 23.2 & 33.0 & 24.6 & 34.0 & 25.9 \\ \hline

% %TAO-VOS & 26.4 & 25.8  & 33.7 & 23.2 \\
% \end{tabular}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\arraystretch{1.35}
\setlength\tabcolsep{2.4pt}
 
\resizebox{0.47\textwidth}{!}{
\begin{tabu}{c cccc}
\tabucline[1pt]{-}
 \multirow{2}{*}{Dataset}&  \multicolumn{2}{c}{\textbf{Fusion Layer5}} & \multicolumn{2}{c}{\textbf{Fusion Layer2}}    \\
\cline{2-5}
  & Dyn.(\%) & Stat.(\%)& Dyn.(\%) & Stat.(\%)\\
\tabucline[1pt]{-}
TAO-VOS & 26.4 & 25.8  & 33.7 & 23.2 \\
ImageNetVID & 26.4 & 33.1 & 33.0 & 24.6  \\
DAVIS & 27.8 & 30.1 & 34.0 & 25.9 \\

\tabucline[1pt]{-}
\end{tabu}
%%%%%%%%%%%%%%%%%%%%%%5
\hspace{0.08cm}
\begin{tabular}{c}
\includegraphics[width=0.12\textwidth]{tex/images/saliency_priors/prior2.pdf}
\end{tabular}

}
\end{center}
\vspace{-0.4cm}
\caption{Dynamic and static biases of video object segmentation datasets using the layer-wise metric, (\ref{eq:biasscores}). \textbf{Left}: Encoding of dynamic and static factors for FusionSeg model last sensor fusion layer, trained on \textbf{DAVIS}, \textbf{ImageNetVID} and \textbf{TAO-VOS}. \textbf{Right}: Center bias plots for DAVIS, ImagenetVID and TAO-VOS datasets. The first two datasets have more center bias than TAO-VOS. \textcolor{blue}{Order plots on right in the same order as table entries on the left and adjust the caption correspondingly. Also, the caption says that the LHS shows results for the \textit{last} sensor fusion layer only, while the actual table shows results for that layer and another. As it stands, I've deleted the interpretation and moved it to the text, because it seems a bit more complicated than was tersely stated here.}}\label{fig:vos_dataset}
\end{figure}

==> core/graphs/vos_iterwise.tex <==
\begin{figure}
\begin{tikzpicture}[trim axis left,trim axis right]\ref{target_legend7}
    \begin{axis}[
      line width=1.0,
        title={MATNet - (DAVIS+YTB)},
        title style={at={(axis description cs:0.5,0.9)},anchor=north,font=\normalsize},
        xlabel={Epoch},
        x label style={font=\small},
        ylabel={Number of Units (\%)},
        xmin=-1, xmax=200,
        ymin=15, ymax=40,
        xtick={20,40,60,80,100,120,140,160,180},
        ytick={20, 25, 30, 35, 40},
        % yticklabels={,,},
        x tick label style={font=\tiny, rotate=0, anchor=north},
        y tick label style={font=\tiny},
        x label style={at={(axis description cs:0.5,0.1)},anchor=north,font=\small},   
        y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},        width=6.5cm,
        height=4.3cm, % height=4.3cm,   
        ymajorgrids=false,
        xmajorgrids=false,
        major grid style={dotted,green!20!black},
        legend columns=2,
        legend style={
        % mark options={scale=0.1}
         nodes={scale=0.6, transform shape},
         cells={anchor=west},
         legend style={at={(1.9,0.0)},anchor=south,row sep=0.01pt}, font =\normalsize},
         legend entries={[black]Fusion2Static,[black]Fusion5Static,[black]Fusion2Dynamic,[black]Fusion5Dynamic},
        legend to name=target_legend7,
    ]
   %
    \addplot[line width=1.2pt,mark size=1.1pt,color=cyan]
        coordinates {(0,20.0)(5,22.5)(10,23.3)(15,25.0)(25,24.5)(45,26.5)(50,25.4)(60,28.5)(75,23.8)(80,24.4)(85,24.7)(90,24.7)(95,26.0)(105,24.7)(110,24.3)(115,23.7)(120,24.3)(125,23.7)(130,25.5)(140,24.1)(145,23.0)(150,23.5)(155,24.6)(160,24.1)(165,23.9)(170,24.3)(175,24.2)(180,23.4)(185,24.1)(190,24.0)};
    % APPEARANCE
    \addplot[line width=1.2pt,mark size=1.1pt,color=orange]
        coordinates {(0,39.6)(5,35.9)(10,23.3)(15,25.0)(25,34.0)(45,29.1)(50,30.7)(60,28.3)(75,34.0)(80,33.4)(85,32.5)(90,32.5)(95,31.4)(105,31.7)(110,31.1)(115,33.9)(120,33.7)(125,34.5)(130,31.1)(140,33.9)(145,33.3)(150,33.9)(155,32.7)(160,32.9)(165,33.4)(170,33.0)(175,32.8)(180,33.5)(185,32.9)(190,32.9)};
        % FAST
        % MOTION
    \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=cyan]
        coordinates {(0,22.3)(5,25.8)(10,27.3)(15,28.5)(25,27.7)(45,32.0)(50,31.2)(60,29.7)(75,28.5)(80,30.9)(85,31.6)(90,31.6)(95,32.8)(105,29.3)(110,31.6)(115,31.2)(120,33.6)(125,33.6)(130,31.2)(140,30.5)(145,30.9)(150,32.0)(155,32.4)(160,30.5)(165,31.2)(170,30.9)(175,30.1)(180,30.1)(185,30.9)(190,29.7)};
    % APPEARANCE
     \addplot[densely dotted,line width=1.2pt,mark size=1.1pt,color=orange]
        coordinates {(0,38.3)(5,32.4)(10,27.0)(15,25.0)(25,27.0)(45,23.0)(50,23.4)(60,22.7)(75,21.9)(80,21.9)(85,22.7)(90,20.7)(95,20.7)(105,21.9)(110,23.0)(115,23.4)(120,21.9)(125,22.3)(130,20.7)(140,22.7)(145,22.7)(150,21.9)(155,22.7)(160,22.7)(165,22.7)(170,21.1)(175,21.9)(180,23.4)(185,22.3)(190,22.7)};
\end{axis}
\end{figure}
